Efficient Topology-Controlled Sampling of Implicit Shapes

Sampling from distributions of implicitly defined shapes enables analysis of various energy functionals used for image segmentation. Recent work describes a computationally efficient Metropolis-Hastings method for accomplishing this task. Here, we extend that framework so that samples are accepted at every iteration of the sampler, achieving an order of magnitude speed up in convergence. Additionally, we show how to incorporate topological constraints.

==> background.tex <==
In this section, we briefly review some concepts and related work that are relevant to the scope of this thesis.

\subsection{Shape Sampling}
Level-set based segmentation is often formulated as an energy minimization problem, where some energy functional is chosen such that a ``good'' segmentation occurs at low energies. It is often the case that, either due to the ill-posedness of unsupervised segmentation or the stochastic nature of a well posed formulation, multiple plausible explanations exist. For example, consider the expert segmentations shown in Figure \ref{fig:human-segs}.
\begin{figure}
	\centering
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090_1}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090_2}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090_3}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090_4}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.16\linewidth]{figures/143090_5}}\vspace*{-7pt}%
	\caption{Example expert segmentations from \cite{Martin2001}. The original image is shown on the left.}
	\label{fig:human-segs}
\end{figure}
In some cases, the reflection of the island is assigned its own label while in others, it is grouped with the water. In cases such as these, characterization of the posterior distribution of segmentations may offer a more informative solution to the problem. Consequently, a common alternative to the minimization formulation is to recast the problem as one of Bayesian inference, where the energy functional is viewed as the negative log of the posterior distribution of labels conditioned on data:
\begin{equation}
	p(\ell \vert x) \propto \exp (-E(\ell; x)),
	\label{eqn:energy}
\end{equation}
where $\ell$ is the matrix of labels assigned to each pixel (i.e. the segmentation) and $x$ is the set of data values at each pixel.

Sampling from the space of implicit segmentations has been suggested previously. Fan et al. \cite{Fan2007} develop a hybrid method: alternating between implicit (level set) and explicit (marker based) representations of a simply connected shape. The proposal distribution generates a sample perturbation over a set of marker points which, when computing the \textit{Hastings ratio}, induces a correspondence problem over the explicit representation. Upon completion, the new sample is converted into an implicit form by resolving the Eikonal equation. While establishing the feasibility of applying MCMC methods to implicit representations, \cite{Fan2007} is constrained to binary segmentations of a single, simply connected shape. Furthermore, iterations between implicit and explicit representations incur a substantial computational burden. Fan suggests the use of jump diffusion processes \cite{Grenander1998} as a means of incorporating topological changes. However, no formulation satisfying detailed balance is provided.

Chen et al. \cite{Chen2009} improve upon the method of Fan et al. by obviating the need to transition between implicit and explicit representations. They construct a smooth normal perturbation at a \textit{single} point on the curve (denoted the ``foot point") that preserves the signed distance property between proposal samples, thereby simplifying the correspondence problem and evaluation of the Hastings ratio. However, the resulting perturbations are extremely smooth, and as such, explore the configuration space very slowly. As in \cite{Fan2007} obstacles remain for incorporating topological changes, restricting this method to binary segmentations with a single simply connected shape. Preliminary results shown in Section \ref{sect:TC-BFPS} indicate that significant computational gains combined with a more expressive model are possible.





\subsection{Digital Toplogy and Constrained Level-Set Evolution}
The topology of a continuous, compact surface is often described by its genus (i.e. the number of ``handles''). Homeomorphisms are deformations of such a surface that preserve the genus (e.g. stretching, bending, twisting, etc.).  Digital topology \cite{Rosenfeld1981} \cite{Kong1989} is the discrete counterpart of continuous topology, where regions are represented via binary variables on a grid.

In digital topology, one needs to first define a \textit{connectiveness} for the foreground and background, which describes how pixels in a local neighborhood are ``connected''. For example, in 2D, a 4-connected region corresponds to a pixel being connected to its neighbors above, below, left, and right. An 8-connected region corresponds to a pixel being connected to the eight pixels in a 3x3 neighborhood. Connectiveness must be jointly defined for the foreground ($n$) and background ($\overline{n}$) to avoid topological paradoxes. For example, consider the configurations shown in Figure \ref{fig:topological-paradoxes}.
\begin{figure}
	\centering
	\subfloat[$(n,\overline{n})=(8,8)$]{\hspace*{20pt}\includegraphics[width=0.2\linewidth]{figures/topological_paradox1}\hspace*{20pt}}\hspace*{5pt}%
	\subfloat[$(n,\overline{n})=(4,4)$]{\hspace*{20pt}\includegraphics[width=0.2\linewidth]{figures/topological_paradox2}\hspace*{20pt}}\hspace*{5pt}%
	\subfloat[$(n,\overline{n})=(4,8)$]{\hspace*{20pt}\includegraphics[width=0.2\linewidth]{figures/topological_paradox3}\hspace*{20pt}}\vspace*{-7pt}
	\caption{Examples of connectiveness. The first two, $(8,8)$ and $(4,4)$ correspond to topological paradoxes where portions of the image are represented by either both foreground and background or neither.}
	\label{fig:topological-paradoxes}
\end{figure}
if the foreground and background are both 8-connected, the implicit curves have a possibility of overlapping. If both regions are 4-connected, the implicit curves will not span the entire space. As shown in \cite{Kong1989}, valid connectivities for 2D are $(n,\overline{n})\in\left\{(4,8), (8,4)\right\}$.

Given a pair of connectiveness for the foreground and background (e.g. $(n,\overline{n})=(4,8)$ in 2D), the topological numbers \cite{Bertrand1994} at a particular pixel, $T_n$ and $T_{\overline{n}}$ correspond to the number of separate regions of the foreground and background the pixel is connected to. Figure \ref{fig:topological-numbers} shows a few 3x3 regions with their corresponding toplogical numbers. A simple point is defined to be a point that, when changed, does not correspond to a topological change. Thus, a homeomorphism in the digital domain can be thought of as a deformation that only changes simple points. One can show \cite{Bertrand1994} that simple points occur at $T_n=T_{\overline{n}}=1$.
\begin{figure}
	\centering
	\subfloat[$T_4=1$, $T_8=1$]{\includegraphics[width=0.33\linewidth]{figures/BFPS/topological_1}}%
	\subfloat[$T_4=2$, $T_8=2$]{\includegraphics[width=0.33\linewidth]{figures/BFPS/topological_2}}%
	\subfloat[$T_4=2$, $T_8=1$]{\includegraphics[width=0.33\linewidth]{figures/BFPS/topological_3}}\vspace*{-7pt}
	\caption{Examples of topological numbers with $(n, \overline{n})=(4,8)$, with $+$ denoting foreground, and $-$ denoting background.}
	\label{fig:topological-numbers}
\end{figure}

The pioneering work of \cite{Han2003} alters the curve evolution gradient velocity point-by-point to not allow any topological changes. If the velocity at a pixel $i$ changes the sign of the height, and the pixel is not a simple point, then the velocity is altered to no longer change the sign. The authors of \cite{Segonne2008} extend the work by allowing certain topological changes like merging and splitting of regions. They define two additional topological numbers, $T_n^+$ and $T_{\overline{n}}^+$, which are the number of unique connected components of the foreground and background respectively. We distinguish these two methods by referring to the work of \cite{Han2003} as single-topology methods (i.e. constrained to a single, specific topology) and \cite{Segonne2008} as topologically-controlled (i.e. controlled evolution within a set of allowable topological changes). 







\subsection{\label{sect:segmentation_measures}Segmentation Scoring}

Because of the ill-posed nature of segmentation \cite{Marroquin1987}, multiple plausible segmentations can exist for a single image. For example, consider the human segmentations shown in Figure \ref{fig:BFPS}. Though there are many similarities across the solutions, discrepancies occur near the boundaries of objects, from the illusory edges, and are a result of the granularity of the segmentation. These varying solutions pose a very important question in segmentation: how does one evaluate the performance of a segmentation algorithm across the \textit{set} of ground truth images?

The Berkeley Segmentation Dataset (BSDS) \cite{Martin2001} attempts to address this question. The dataset consists of a set of 300 images (100 test images, and 200 training images), each of which have been segmented by multiple experts. Additionally, an evaluation criterion for boundary detection using precision-recall curves was developed to score algorithms \cite{Martin2004}. While the precision-recall curves may accurately assess the performance of a boundary detector, it is usually not a good measure of region-based segmentation algorithms. For example, consider the segmentations in Figure \ref{fig:boundary-vs-segmentation}.
\begin{figure}[h]
	\centering%
	\subfloat{\includegraphics[width=0.3\linewidth]{figures/segmeasures/boundary_vs_segmentation_1}}\hspace*{3pt}%
	\subfloat{\includegraphics[width=0.3\linewidth]{figures/segmeasures/boundary_vs_segmentation_2}}
	\caption{An example of how segmentations can differ greatly even when boundary detection is similar. Colors indicate segmentation labels.}
	\label{fig:boundary-vs-segmentation}
\end{figure}
While the boundaries in these two segmentations differ only by a small amount (the strait connecting the two regions), the segmentations are quite different. Boundary detection evaluation methods are clearly not suited to evaluate segmentations. In the following sections, we discuss a few methods on scoring segmentations.

\subsubsection{Probabilistic Rand Index}
One popular way to compare the agreement between two segmentations is by using the Rand Index (RI) \cite{Rand1971}. If a pair of pixels, $\{i,j\}$, was drawn at random from the image domain, the RI finds the empirical expected value of this pair agreeing across both segmentations, $\ell^t$ and $\ell^k$. Mathematically, it can be expressed as
\begin{equation}
	\RI = \hat{\mathbf{E}}_{i,j}\left[ g_{i.j}\left(\ell^t, \ell^k\right) \right] = \frac{1}{\tbinom{N}{2}}\sum_{\{i,j\}} g_{i,j}\left(\ell^t, \ell^k\right),
\end{equation}
where $N$ is the number of pixels in the image, the notation $\sum_{\{i,j\}}$ means the sum over all possible pairs of pixels, $\{i,j\}$, and the agreement is defined as the following
\begin{equation}
	g_{i,j}\left(\ell^t, \ell^k\right)
	= \indicator{\ell_i^t=\ell_j^t}\indicator{\ell_i^k=\ell_j^k}
	 + \indicator{\ell_i^t\neq\ell_j^t}\indicator{\ell_i^k\neq\ell_j^k}.
\end{equation}

Given an algorithm's segmentation result, $\ell^t$, the performance of the algorithm could be scored by considering the Rand Index between $\ell^t$ and one ground truth segmentation, $\ell^k$. However, as stated previously, image segmentation is an ill-posed problem, and results should be evaluated across a \textit{set} of ground truth segmentations. This led to the development of the Probabilistic Rand Index (PRI) \cite{Unnikrishnan2005} and the Normalized Probabilistic Rand Index (NPRI) \cite{Unnikrishnan2005a}, which is an unbiased and normalized version of the PRI. The PRI is essentially the average Rand Index over a set ground truth segmentations, $\left\{\ell^1, \ell^2, ..., \ell^K\right\}$, which we denote as $\ell^{1...K}$:
\begin{equation}
	\PRI = \frac{1}{K}\sum_k \RI
\end{equation}

\subsubsection{Variation of Information}
The variation of information \cite{Meila2003} is an information theoretic evaluation criterion that tries to capture the amount of information that is different between two clusters (or equivalently, segmentations). The variation of information can be written in the following ways:
\begin{align}
	VI(\ell^t, \ell^k)
	&= H(\ell^t) + H(\ell^k) - 2I(\ell^t;\ell^k)\\
	&= H(\ell^t \vert \ell^k) + H(\ell^k \vert \ell^t),
\end{align}
where $H(\cdot)$ is the entropy, $I(\cdot)$ is the mutual information, and $H(\cdot\vert\cdot)$ is the conditional entropy. Figure \ref{fig:vofi} shows the quantities of the variation of information graphically.
\begin{figure}
	\centering%
	\includegraphics[width=0.4\linewidth]{figures/segmeasures/vofi}
	\caption{A graphical representation of the quantities in the variation of information.}
	\label{fig:vofi}
\end{figure}
The first conditional entropy term captures the amount of information in the test segmentation, $\ell^t$, not contained in the ground truth segmentation, $\ell^k$. The second conditional entropy term captures the amount of information in the ground truth segmentation not contained in the test segmentation.

\subsubsection{Global/Local Consistency Error}
While creating the BSDS, the authors also introduced two segmentation measures called the Global Consistency Error (GCE) and the Local Consistency Error (LCE) \cite{Martin2001}. They attempt to capture different granularities of a segmentation by assuming there is a hierarchy of groupings. A segmentation at any granularity should have minimal error. By defining the region of a segmentation to be the set of pixels containing one label
\begin{equation}
	R^t_l = \left\{j; \ell^t_j=l\right\},
\end{equation}
one can define the local refinement error as
\begin{equation}
	E(\ell^t,\ell^k,i) = \frac{\sizeof{R^t_{\ell^t_i}\setminus R^k_{\ell^k_i}}}{\sizeof{R^t_{\ell^t_i}}},
\end{equation}
which attempts to capture a hierarchical-invariant error measure. Using this notion, the GCE and LCE are defined to be:
\begin{align}
	GCE(\ell^t,\ell^k) &= \frac{1}{\sizeof{\Omega}} \min \left\{ \sum_{i\in\Omega} E(\ell^t, \ell^k,i) \,,\,\, \sum_{i\in\Omega} E(\ell^k, \ell^t,i) \right\}\\
	LCE(\ell^t,\ell^k) &= \frac{1}{\sizeof{\Omega}} \sum_{i\in\Omega} \min \left\{ E(\ell^t, \ell^k,i) \,,\,\, E(\ell^k, \ell^t,i) \right\}
\end{align}
As the authors point out, a segmentation containing a single label (i.e. all pixels contained in one region), or a segmentation containing $\sizeof{\Omega}$ labels (i.e. all pixels having different labels) both incorrectly evaluate to zero error under the GCE and LCE.





\begin{comment}
\subsection{Learning Features}
Two important concepts when trying to learn feature extractors from images are the recent deveopments in learning deep Restricted Boltzmann Machines and convolutional networks. We briefly cover these here.

%

\subsubsection{Convolutional Neural Networks}
The first substantial step in learning image descriptors was a result of convolutional neural networks \cite{LeCun1989}. CNNs are a very specific form of neural networks with many connections and only a few weights. They are set up in such a way that the learned weights equivalently act as a convolutional filter on an image. In typical CNNs, the weights of the filter (i.e. the filter coefficients) are learned in a supervised fashion using backpropagation to minimize some surrogate energy.

Commonly in CNNs, each layer of the neural network is composed of a convolutional layer and a sub-sampling or pooling layer. In classification problems, it has been shown \cite{Jarrett2009} that the learning of pooling layers is much more important. With the use of random filters (as compared to learned ones), classification performance only slightly decreases. However, typical CNNs must be trained in a supervised fashion. While recent work (e.g. Ranzato et al. \cite{Ranzato2006}) has developed an unsupervised learning algorithm for CNNs, they are still subject to the particular surrogate function to minimize over. Additionally, as we will see, CNNs are analytical (as opposed to generative) models, which limits its utility.

\subsubsection{Restricted Boltzmann Machines}
A Restricted Boltzmann Machine (RBM) is a single layer within a deep RBM. An RBM consists of a set of ``visible'' variables (denoted $\vect{v}$) and a set of ``hidden'' variables (denoted $\vect{h}$). For computational reasons, a typical RBM models the visible variables as being conditionally independent given the hidden variables and the hidden variables being conditionally independent given the visible variables. An example of this RBM structure is shown in Figure \ref{fig:RBM}. The weight between each node is denoted $w_{ij}$ where $i$ indexes an observed node and $j$ indexes a hidden node.
\begin{figure}[h]
	\centering%
	\includegraphics[scale=0.9]{figures/learning/RBM}
	\caption{An example of a typical RBM.}
	\label{fig:RBM}
\end{figure}

The RBM is typically governed by an energy functional that depends on the weights of the edges (which can be viewed as parameters of the model) and both the visible and hidden variables. In Bayesian methods, it is often convenient to view the negative exponentiated energy functional as being proportional to the likelihood:
\begin{equation}
	P(\vect{v}, \vect{h}; W) \propto \exp\left[-E(\vect{v}, \vect{h}; W)\right]
	\label{eqn:penergy}
\end{equation}
Particular choices of the energy functionals can lead to simpler inference and sampling. For example, one choice of the energy functional is
\begin{equation}
	E(\vect{v}, \vect{h}; W) = \frac{1}{2}\sum_i v_i^2 - \sum_{i,j} v_i w_{ij} h_j - \sum_j b_j h_j - \sum_i c_i v_i,
	\label{eqn:energy}
\end{equation}
where $\mathbf{b}$ and $\mathbf{c}$ are associated biases for the hidden and visible variables respectively. In this particular case, conditioned on the hidden variables, the visible variables are independent and Gaussian. Additionally, conditioned on the visible variables, the hidden variables are independent Bernoulli random variables.

Most energy functionals embed an independence structure; in these cases, we can write the posterior of the visible variables as follows:
\begin{equation}
	P(\vect{v}\vert\vect{h} ; W) = \frac{\prod_j P(\vect{v}\vert h_j ; \vect{w_j})}{\sum_{\vect{v}'\in\mathbb{V}}\prod_j P(\vect{v}'\vert h_j ; \vect{w_j})  },
\end{equation}
where $\mathbb{V}$ is the set of all possible values of $\vect{v}$. The log likelihood is
\begin{equation}
	\log P(\vect{v}\vert\vect{h} ; W) = \sum_j \log P(\vect{v}\vert h_j ; \vect{w_j}) - \log \sum_{\vect{v}'\in\mathbb{V}}\prod_j P(\vect{v}'\vert h_j ; \vect{w_j}).
\end{equation}

One would like to learn the weights, $W$ that maximize the likelihood of the \textit{observed}, visible variables. This maximum likelihood (ML) parameter estimate can be expressed as:
\begin{equation}
	W^\ast = \arg\max_{W} \left[\prod_{\vect{\obs{v}}\in\obs{V}} P(\vect{\obs{v}} \vert \vect{h}; W)\right] = \arg\max_{W} \left[\sum_{\vect{\obs{v}}\in\obs{V}} \log P(\vect{\obs{v}} \vert \vect{h}; W)\right],
\end{equation}
where $\vect{\obs{v}}$ is the vector of one observed, visible variables, and $\obs{V}$ is the set of all observed, visible variables. This estimate can equivalently be expressed as the empirical expected value of the log likelihood taken over the observed, visible variables
\begin{equation}
	W^\ast = \arg\max_{W} \E[\obs{V}]{ \log P(\vect{\obs{v}} \vert \vect{h}; W)}.
\end{equation}
This optimization can be approximately found using gradient ascent. The gradient of the log likelihood for one observation is
\begin{align}
	\frac{\partial \log P(\vect{\obs{v}} \vert \vect{h}; W)}{\partial w_{ij}}
	& = \frac{\partial \log P(\vect{\obs{v}}\vert h_j ; \vect{w_j})}{\partial w_{ij}} - \sum_{\vect{v}\in\mathbb{V}} P(\vect{v}\vert \vect{h} ; W)\frac{\partial \log P(\vect{v}\vert h_j ; \vect{w_j})}{\partial w_{ij}}\\
	& = \frac{\partial \log P(\vect{\obs{v}}\vert h_j ; \vect{w_j})}{\partial w_{ij}} - \E[\mathbb{V}]{\frac{\partial \log P(\vect{v}\vert h_j ; \vect{w_j})}{\partial w_{ij}}}
	\label{eqn:dloglikelihood}
\end{align}
Thus, the entire gradient over all observations (combined with Equations \ref{eqn:penergy} and \ref{eqn:energy}) is
\begin{align}
	\frac{\partial \E[\obs{V}]{\log P(\vect{\obs{v}} \vert \vect{h}; W)}}{\partial w_{ij}}
	& = \E[\obs{V}]{\frac{\partial \log P(\vect{\obs{v}}\vert h_j ; \vect{w_j})}{\partial w_{ij}}} - \E[\mathbb{V}]{\frac{\partial \log P(\vect{v}\vert h_j ; \vect{w_j})}{\partial w_{ij}}}\\
	& = \E[\obs{V}]{\obs{v}_i h_j} - \E[\mathbb{V}]{v_i h_j}.
	\label{eqn:dloglikelihood}
\end{align}

The expectations in the above equation can be estimated using samples from the distributions. Because the observed variables are conditionally independent given the hidden variables (and vice versa), we can perform block Gibbs sampling to draw samples from the joint:
\begin{enumerate}
	\item Iteration $0$:
		\begin{enumerate}
			\item Set the observed variables to be the actual observation: $\vect{v}^{(0)}=\vect{\obs{v}}$
			\item Draw a set of hidden variables from the posterior: $\left\{h_j^{(0)} \sim P(h_j\vert\vect{v}^{(0)} ; W^{(0)})\right\}$
		\end{enumerate}
	\item Iteration $n>0$:
		\begin{enumerate}
			\item Draw a set of observed variables from the posterior: $\left\{v_i^{(n)} \sim P(v_i\vert\vect{h}^{(n)} ; W^{(n)})\right\}$
			\item Draw a set of hidden variables from the posterior: $\left\{h_j^{(n)} \sim P(h_j\vert\vect{v}^{(n)} ; W^{(n)})\right\}$
		\end{enumerate}
\end{enumerate}
The first term in Equation \ref{eqn:dloglikelihood}, $\E[\obs{V}]{\obs{v}_i h_j}$ can be estimated from samples from iteration 0, and the esecond term, $\E[\mathbb{V}]{v_i h_j}$ can be estimated from samples from iteration $\infty$ as follows:
\begin{equation}
	\frac{\partial \E[\obs{V}]{\log P(\vect{\obs{v}} \vert \vect{h}; W)}}{\partial w_{ij}} = \left\langle v_i^{(0)} \, h_j^{(0)}\right\rangle - \left\langle v_i^{(\infty)} \, h_j^{(\infty)}\right\rangle,
\end{equation}
where $\langle\cdot\rangle$ denotes the sample average. It can be shown that the gradient of the log likelihood is equivalent to the gradient of the following negative KL divergence:
\begin{equation}
	\frac{\partial \E[\obs{V}]{\log P(\vect{\obs{v}} \vert \vect{h}; W)}}{\partial w_{ij}} = \frac{\partial D\left(\vect{\obs{v}} \Vert \vect{v} \right) } {\partial w_{ij}} = \frac{\partial D\left(\vect{v}^{(0)} \Vert \vect{v}^{(\infty)} \right) } {\partial w_{ij}}
\end{equation}
In practice, waiting for the Markov chain to converge can take a long time. Thus, minimizing contrastive divergence \cite{Hinton2002} is typically used as an approximation:
\begin{equation}
	\frac{\partial \left(D\left(\vect{v}^{(0)} \Vert \vect{v}^{(1)} \right) - D\left(\vect{v}^{(1)} \Vert \vect{v}^{(\infty)} \right)\right) } {\partial w_{ij}} = \left\langle v_i^{(0)} \, h_j^{(0)}\right\rangle - \left\langle v_i^{(1)} \, h_j^{(1)}\right\rangle.
\end{equation}

\subsubsection{Learning in Deep Networks}
One typically stacks multiple layers of RBMs on top of each other to learn a hierarchical set of features. The lower level RBMs can then typically learn low level features, while higher level RBMs can combine these features to identify higher level features. While training a single layerered RBM is straightforward, reliably training these deep belief networks can be difficult. Hinton et al. \cite{Hinton2006a} proposed a greedy layer-wise training algorithm that performs well in practice.

\subsubsection{Convoluational RBMs}
While deep belief networks (DBNs) consisting of mulitple layers of RBMs have shown considerable success in small image tasks (e.g. \cite{Hinton2006a}), they do not scale well with image size. There has been some more recent work \cite{Lee2009,Desjardins2008} on convolutional deep belief networks, where each layer consists of a small RBM that is applied at every location to the image. These convolutional RBM (CRMB) layers can be thought of as sharing weights between visible and hidden variables across the entire image. The weights are constrained in such a way they equivalently produce a convolution on a layer of nodes. Figure \ref{fig:CRBM} shows an example of tied weights that perform a one-dimensional convolution of support three.
\begin{figure}
	\centering
	\includegraphics[scale=0.9]{figures/learning/CRBM}
	\label{fig:CRBM}
	\caption{An example of tied weights that perform a finite one-dimensional convolution of support three. Each unique weight is represented with a different line (double, single, or dotted).}
\end{figure}
These generative models have shown encouraging results on recognition and other computer vision tasks.
\end{comment}

==> mary.tex <==
The previous section described the binary GIMH sampling scheme. Similar to the BFPS algorithm \cite{Chang2011}, we can extend the GIMH to an $M$-ary segmentation sampling scheme. We begin with a brief review the M-ary framework of BFPS.

BFPS builds on the framework of \cite{Brox2006} which represents each unique region with one level-set. However, instead of using $M$ level sets for $M$ regions, BFPS uses $(M-1)$ level-sets. The support of region $m$, $R_m$, is represented with the positive pixels of the $m^{\text{th}}$ level-set:
\begin{equation}
 	R_m = \left\{i \vert \varphi_m(i)\geq 0\right\},
\end{equation}
where $m\in[1,\dots,M-1]$. The support of the remaining region, denoted the \textit{null} region, is represented as the intersection of all negative pixels:
\begin{equation}
	R_0 = \cap_{m} \left\{i \vert \varphi_m(i) < 0 \right\}.
\end{equation}

As with most $M$-ary representations, one needs to ensure that vacuum and overlap conditions \cite{Brox2006} do not occur. A vacuum condition, where a pixel in the image is not represented with any region, is implicitly restricted by the null region representation. On the other hand, an overlap condition, where a pixel in the image is represented by more than one region, needs to be explicitly enforced by the proposal. At each iteration in the proposal, a particular level-set function, $\varphi_m$, is first selected at random. The additive BFPS proposal distribution is modified so that perturbations at each iteration only acts on pixels within $R_m \cup R_0$.

With this formulation, a pixel moving from region $R_{m_1}$ to $R_{m_2}$ must first temporarily move to region the null region, $R_0$. This complication required the alteration of the bias in the proposal; instead of using the gradient velocity, BFPS uses what was denoted as the \textit{minimal} gradient velocity. While these two modifications allow one to sample $M$-ary implicit shapes, they often led to slower convergence. Additionally, the sampling procedure may converge to local extrema with particular initializations. For example, consider the image and corresponding initialization shown in Figure \ref{fig:BFPS-MARY}. This figure illustrates the required moves that pixels must make to transition to the correct label. This is accomplished in two steps: (1) pixels that are initially incorrectly grouped with the circle must first transition to the null (background) region, and (2) the pixels must transition from the null region to the correct square region. The problem with this lies in the first transition. Because this is an MCMC Metropolis-Hastings procedure, one must first accept the proposal to transition from the circle to the null region. However, because the pixel intensities are more similar to the circle than the background, this proposal will almost surely be rejected. The BFPS framework will potentially get stuck in these types of local extrema if multiple restarts are not used.
\begin{figure}
	\centering
	\begin{minipage}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/BFPS_1}\\\vspace*{50pt}
	\end{minipage}
	\begin{minipage}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/BFPS_2}\\\vspace*{2pt}
		\includegraphics[width=\linewidth]{figures/BFPS_2r}\\
		Initialization
	\end{minipage}
	\begin{minipage}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/BFPS_3}\\\vspace*{2pt}
		\includegraphics[width=\linewidth]{figures/BFPS_3r}\\
		Move to Null Region
	\end{minipage}
	\begin{minipage}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/BFPS_4}\\\vspace*{2pt}
		\includegraphics[width=\linewidth]{figures/BFPS_4r}\\
		Move to Correct Region
	\end{minipage}
	\label{fig:BFPS-MARY}
	\caption{Illustrating the necessary moves for $M$-ary BFPS to transition to the correct segmentation.}
\end{figure}

In this work, we instead use $M$ level-set functions to represent $M$ regions. We formulate a simple representation that ensures no vacuum or overlap conditions without having to greatly alter the proposal distribution. Each pixel $i$ belongs to the region that has the highest height:
\begin{equation}
	R_m = \left\{ i \; \Big\vert \; m = \arg\max_\ell \varphi_\ell(i) \right\}.
\end{equation}
This representation ensures that each pixel belongs to one and only one region. The associated proposed perturbation is similar in that a constant is added to a random mask of pixels. However, the ranges and proposal over ranges (Equation \ref{eqn:proposal-range}) must be altered to correctly represent the target distribution.

We define the difference between to level sets to be
\begin{equation}
	\Delta_i(\varphi_{\ell_1}, \varphi_{\ell_2}) = \varphi_{\ell_1}(i) - \varphi_{\ell_2}(i),
\end{equation}
the maximal level-set at pixel $i$ to be
\begin{equation}
	\varphi_{\max}(i) = \varphi_{\arg\max_\ell \varphi_\ell (i)}.
\end{equation}
Additionally, as we shall see, we will need the second largest level-set at each pixel which we define as $\max^2 \varphi_\ell(i)$. The resulting second maximal level-set at pixel $i$ can then be written as
\begin{equation}
	\varphi_{\max^2}(i) = \varphi_{\arg\max^2_\ell \varphi_\ell (i)}.
\end{equation}
We use this notation in defining the extent of each range, which is no longer just the height of the level-set function. We remind the reader that a particular level-set, which we call the \textit{perturbing level-set}, $\varphi_m$, is first selected as the one to perturb. A pixel, $i$, belongs to region $R_m$ if it has the maximal height among all level-set functions (i.e. $\varphi_m(i) \equiv \varphi_{\max}(i)$). For such a pixel, $i$, to change regions, we must subtract at least as much height as $\Delta_i(\varphi_m, \varphi_{\max^2})$ (the difference between the perturbing level-set and the second maximum height). On the other hand, for a pixel that currently does not belong to a region $R_m$ to change, we must add at least as much height as $\Delta_i(\varphi_{\max}, \varphi_m)$ (the difference between the maximum and the perturbing level-set height). An example of the range endpoints is shown in Figure \ref{fig:mary-ranges} for $M=2$.
\begin{figure}
	\centering
	\subfloat{\includegraphics[scale=1]{figures/mary_mask_distributions1}}\hspace*{10pt}
	\subfloat{\includegraphics[scale=1]{figures/mary_mask_distributions2}}
	\caption{$M$-ary range description for $M=2$. A random mask is shown on the left, with pixel locations marked by the suit symbols: $\clubsuit \vardiamond \varheart \spadesuit$. On the right, the height of each of the pixels is plotted on the real line for two level-set functions, $\varphi_m$ and $\varphi_{\overline{m}}$. The possible ranges for the perturbing level-set, $\varphi_m$, are shown above these plots, where the dotted line is the zero-perturbation line.}
	\label{fig:mary-ranges}
\end{figure}
BFPS allowed pixels to move from $R_0 \rightarrow R_m$ or $R_m \rightarrow R_0$. This representation allows pixels to move from $R_{\max} \rightarrow R_m$ or $R_m \rightarrow R_{\max^2}$, where $R_{max}$ and $R_{max^2}$ could potentially be any other region, not just $R_0$. For this reason, local extrema situations like the one shown in Figure \ref{fig:BFPS-MARY} do not affect this representation. As a demonstration, we show part of one sample path GIMH-SS framework in Figure \ref{fig:GIMH-MARY}.
\begin{figure}
	\centering
	\subfloat{\includegraphics[width=0.19\linewidth]{figures/BFPS_1}}\hspace*{2pt}
	\subfloat{\includegraphics[width=0.19\linewidth]{figures/GIMH2}}\hspace*{2pt}
	\subfloat{\includegraphics[width=0.19\linewidth]{figures/GIMH3}}\hspace*{2pt}
	\subfloat{\includegraphics[width=0.19\linewidth]{figures/GIMH4}}\hspace*{2pt}
	\subfloat{\includegraphics[width=0.19\linewidth]{figures/GIMH5}}\\\vspace*{-7pt}
	\subfloat{\makebox[0.19\linewidth][c]{Original}}\hspace*{2pt}
	\subfloat{\makebox[0.19\linewidth][c]{Initialization}}\hspace*{2pt}
	\subfloat{\makebox[0.4\linewidth][c]{Intermediate Iterations}}\hspace*{2pt}%
	\subfloat{\makebox[0.19\linewidth][c]{Final Sample}}\\%[\beforeCapt]%
	\caption{An example of $M$-ary GIMH-SS with an intialization that causes problems in BFPS.}
	\label{fig:GIMH-MARY}
\end{figure}

This $M$-ary framework is also closely-related to the binary framework. In the binary case, perturbations to the level-set changed pixels so that they were either positive or negative valued. In the $M$-ary case, the perturbation to a particular level-set changes pixels so that they are either the maximal value or not the maximal value. In fact, this $M$-ary framework simplifies to the binary framework if $M=2$, $\varphi_2(i)=0 \quad \forall i$, and the perturbing level-set is always chosen to be $\varphi_1$.



==> shape_sampling.tex <==
In this section, we develop an efficient Metropolis Hastings MCMC sampler to sample from these distributions. We additionally show how to extend the topologically controlled evolution of \cite{Segonne2008} and \cite{Han2003} to a proposal distribution while satisfying detailed balance. As argued by \cite{Han2003}, when the topology of the underlying object is known, restricting the segmentation to such a constraint can drastically improve results in noisy images and when occlusions exist.

Sampling from the infinite space of continuous shapes has proven to be a hard problem to solve efficiently. Previous methods (as discussed in Section \ref{sect:background}) use a Metropolis Hastings (MH) Markov chain Monte Carlo (MCMC) sampling scheme. When using these MCMC samplers, one has to wait for a sufficient amount of time for the chain to properly mix into its stationary distribution. As such, random moves in a large space can take a very long time to converge. The methods of \cite{Fan2007} and \cite{Chen2009} both take on the order of days to draw a single sample from the posterior distribution of interest. In this section, we show how to design a proposal distribution in the MH-MCMC sampler to speed up convergence by orders of magnitude. Drawing a single sample via the proposed algorithm takes on the order of minutes. We additionally extend the sampling scheme to M-ary segmentation, and show how to formulate a topology-controlled proposal.

\subsection{\label{sect:BFPS}Biased Filtered Point Sampling}
We begin by developing the basic, binary implicit shape sampler named the Biased Filtered Point Sampler (BFPS). Additional details can be found in \cite{Chang2011}.
\subsubsection{Metropolis-Hastings MCMC Sampling}
One can construct a Metropolis-Hastings sampler \cite{Hastings1970} as follows. Let $\hatlevelset{t+1}$ be a proposed sample of the implicit representation (i.e. the level-set function) generated from a distribution $q(\hatlevelset{t+1} \vert \levelset{t})$ conditioned on the current sample, $\levelset{t}$. The superscript values $\left(t\right)$ and $\left(t+1\right)$ index the sampling iteration and the hat indicates a proposed sample. This new sample is then accepted with probability 
%
\begin{equation}
	\text{Pr}\left[\levelset{t+1} = \hatlevelset{t+1} \,\big\vert\, \levelset{t} \right]
	= \min\Bigg[
\overbrace{\underbrace{\frac{\pi\left(\hatlevelset{t+1}\right)}{\pi\left(\levelset{t}\right)}}_{\text{Posterior Sample Ratio}} \cdot \underbrace{\frac{q\left(\levelset{t} \big\vert \hatlevelset{t+1} \right)}{q\left(\hatlevelset{t+1} \big\vert \levelset{t} \right)}}_{\text{Forward-Backward Ratio}}}^{\text{Hastings Ratio}}
	, 1 \Bigg].
	\label{eqn:metropolis-hastings}
\end{equation}
%
Otherwise, $\levelset{t+1} = \levelset{t}$. Convergence to the stationary distribution occurs after a suitable number of iterations (i.e. the mixing time) which produces a \textit{single} sample from the posterior. Evaluating the Hastings ratio, the product of the two ratios in the acceptance probability, has been the primary barrier for implementing MCMC methods over implicit representations. In particular, one needs to solve a correspondence problem  to compute the probability of generating the forward and reverse transition (in the forward-backward ratio). Doing so satisfies the condition of detailed balance which, in addition to ergodicity, is sufficient for convergence to the desired posterior distribution.

As with any level-set representation, one needs to choose the magnitude of the level-set, $\varphi$, away from the curve. Previous sampling methods have constrained the level-set function to be a signed distance function (SDF). Fan et al. \cite{Fan2007} alternates between an implicit and explicit representation Chen \cite{Chen2009} solves the correspondence problem by generating perturbations that are SDF-preserving, thus having a one-to-one mapping from forward and reverse transitions. An alternative is to produce a non-SDF-preserving perturbation and reinitialize the level set function to an SDF at each iteration. However, this creates a many-to-many correspondence problem which significantly increases the computational complexity of the forward-backward ratio.

Our idea is straightforward: do not constrain the level-set function to be an SDF. SDFs provide advantages in terms of numerical stability and the computation of the curvature (see \cite{Osher2003} for details) for optimization based methods. As the method here is not PDE-based and optimization is not the specific goal, there is essentially no penalty for using an alternative. While our level-set function no longer satisfies the SDF property, we still benefit from the way implicit representations handle topological changes and re-parameterization. Furthermore, this greatly simplifies the design and evaluation of a proposal distribution by allowing for straightforward evaluation of the Hastings ratio.
%
\subsubsection{Strategic Bias in the Proposal Distribution}
%
We note that the closer $q\left(\circ|\triangle\right)$ is to $\pi\left(\circ\right)$, the closer the Hastings ratio is to unity and the higher the acceptance rate. Consequently, designing proposal distributions which capture essential, application-specific characteristics of the posterior distribution can improve convergence speeds by reducing the number of rejected samples. By relaxing the SDF constraint on the level-set function, many potential proposal distributions will result in a tractable evaluation of the Hastings ratio. Without care, however, the majority of these proposal distributions will have very poor mixing times. Thus, our aim is to design a proposal distribution that is easily evaluated, has a high acceptance rate, and explores the configuration space via large perturbations.

In Equation \ref{eqn:metropolis-hastings}, the Hastings ratio consists of the posterior sample ratio (PSR) and the forward-backward ratio (FBR). The PSR represents the ratio of the posterior probability of the new sample over that of the old. Generating samples that have higher posteriors will produce high values of this ratio. The FBR represents the probability of generating the previous sample conditioned on the new one (the backward transition) over the probability of generating the new sample conditioned on the previous one (the forward transition).

Fan et al. \cite{Fan2007} suggest using a proposal distribution biased by the curvature to favor samples that fit the prior model. Here, we develop a proposal which favors both the likelihood and prior model. This generally produces higher PSR values, but biases the FBR toward smaller values (see the supplemental materials for an illustrative example).
%
\begin{comment}
The following example illustrates this point\footnote{see the supplemental materials for an example}.

\highlight{Let us assume that a proposal sample is generated deterministically from $N$ i.i.d. biased Gaussian random variables, $X_1, X_2, ..., X_N \sim \mathcal{N}\left(\mu,\sigma^2\right)$. Here, we treat the FBR as a random variable and explore the distribution of this ratio as a function of $N$ and $\mu$. We define the random variables $Y_i$ and $Z_N$ as}
\begin{equation}
	Y_i = \log\frac{p_X\left(-X_i\right)}{p_X\left(X_i\right)}, \quad 
	Z_N = \sum_{i=1}^N Y_i = \log \left[\text{FBR}\right].
\end{equation}
\highlight{With some manipulation, it can be shown that $Y_i \sim \mathcal{N}\left(-\frac{2\mu^2}{\sigma^2}, \frac{4\mu^2}{\sigma^2}\right)$ and $Z_N \sim \mathcal{N}\left(-\frac{2N\mu^2}{\sigma^2}, \frac{4N\mu^2}{\sigma^2}\right)$. The FBR ratio therefore follows a log-normal distribution, where the distribution of the log of the FBR is just the density of $Z_N$, $p_{Z_N}$. In Figure} \ref{fig:biased-density}\highlight{, we plot the density of $Z_N$ for varying values of $N$, the number of random variables used to generate a proposal, and $\mu/\sigma$, the amount of bias. Clearly, as $N$ or $\mu/\sigma$ increase, proposals with smaller FBRs are \textit{much} more likely to be generated.}
\begin{figure}
	\centering
		\vspace*{-7pt}
	\subfloat{\label{fig:biased-density_N}\includegraphics[width=0.45\linewidth]{figures/pz_n}}\hspace*{10pt}%
	\subfloat{\label{fig:biased-density_SNR}\includegraphics[width=0.45\linewidth]{figures/pz_mu}}
	\caption{Distributions of the FBR for biased proposals as a function of the number of biased RVs ($N$) and the amount of bias ($\mu/\sigma$).}
	\label{fig:biased-density}
\end{figure}
\end{comment}
%
%
%
%
Thus, our goal is to develop a proposal distribution with a higher overall Hastings ratio (the product of the PSR and the FBR), where deleterious effects on the FBR are compensated with increases in the PSR. Exploiting the simple observation that neighboring pixels tend to have the same label, we can develop a proposal that has this property.
%
\begin{comment}
The previous example illustrates the decreasing nature of the FBR from generating samples from a biased proposal distribution. However, as stated previously, we desire to generate proposal perturbations that (1) contain large moves (larger $N$) so that the convergence speed can increase and (2) are biased towards likely samples (larger $\mu/\sigma$) so that the PSR can increase. We abate the inherent tradeoff between increasing the PSR while decreasing the FBR by drawing on the observation that neighbouring pixels in an image tend to have the same label.
\end{comment}
%

We construct an additive perturbation, $\mathbf{f}$, to $\levelset{t}$,
%
\begin{equation}
	\hatlevelset{t+1} = \levelset{t} + \mathbf{f}^{\left(t\right)},
\end{equation}
%
by first sampling from a point process, attributing the points with values sampled from a biased Gaussian distribution and then smoothing with a lowpass filter. We refer to this process as Biased and Filtered Point Sampling (BFPS). The lowpass filter captures the property that pixels in close proximity have higher probability of being in the same region while the \textit{choice} of bias favors points with high likelihood under the energy functional. The result is dramatically increased PSRs using large biased moves while only slightly decreasing the FBR. Mathematically this is expressed as
%
\begin{equation}
	\mathbf{f}^{\left(t\right)} = \mathbf{h}^{\left(t\right)} \ast \left(\mathbf{c}^{\left(t\right)} \circ \mathbf{n}^{\left(t\right)}\right),
\end{equation}
\begin{equation}
	n_i^{(t)}\sim\mathcal{N}\left(\mu_i^{(t)}, \sigma^2\right),\quad
%
%
	c_i^{(t)}\sim\text{Bernoulli}\left(p_{c_i}^{(t)}\right),
\end{equation}
%
where `$\ast$' denotes convolution and `$\circ$' denotes the element-wise product. We bias the Gaussian RVs with the gradient velocity, $\mathbf{v}^{(t)}$, (the negative gradient of the energy functional) to prefer moving to more probable configurations:
\begin{equation}
	\mu_i^{(t)} = \alpha_n \left[-\frac{\partial E\left(\levelset{t}\right)}{\partial \levelset{t}}\right]_i = \alpha_n v_i^{(t)},
	\label{eqn:bias}
\end{equation}
where $\alpha_n$ is a weighting parameter. The probability associated with each point, $c_i$, is also carefully selected to favor selecting points which are better explained in another region. Specifically, it is chosen to be higher for points that have a gradient velocity that is large in magnitude \textit{and} has the opposite sign of the current level-set value:
\begin{equation}
	p_{c_i}^{(t)}(1) \propto \alpha_c \exp\left[ -v_i^{(t)} \cdot \text{sign}\left(\levelset{t}_i\right) \right] + \left(1-\alpha_c\right),
	\label{eqn:pc}
\end{equation}
where $\alpha_c$ is a parameter that trades off the bias with a uniform distribution. Additionally, we define the variable $\gamma$ as $\frac{1}{\sizeof{\Omega}}\sum_{i\in\Omega} p_{c_i}^{(t)}(1)=\gamma$, which approximates the average probability that a random point will be selected, where $\Omega$ is the set of all pixels. Because $p_{c_i}^{(t)}(1)$ is only defined up to a scale factor, we can renormalize its value to achieve any $\gamma$. In practice, $\alpha_n$, $\alpha_c$, and $\gamma$ are dynamically adapted to maintain a minimum acceptance rate, and $\mathbf{h}^{\left(t\right)}$ is chosen to be a circularly symmetric (truncated) Gaussian kernel with a scale parameter randomly chosen from a finite set of values. Randomly chosen scale parameters introduce a minor complication (which we address), but empirically result in faster mixing times.

This algorithm can additionally be extended to M-ary segmentation. Details about the formulation and results obtained using this sampling algorithm can be found in \cite{Chang2011}. An illustration of what this proposal sample looks like is shown in 1D in Figure \ref{fig:1D-BFPS}
\begin{figure}
	\centering
%
	\subfloat[$\levelset{j}$]{\label{fig:biased-density_N}\includegraphics[width=0.2\linewidth]{figures/BFPS/phi}}\hspace*{5pt}%
	\subfloat[$f^{(j)}$]{\label{fig:biased-density_N}\includegraphics[width=0.2\linewidth]{figures/BFPS/f}}\hspace*{5pt}%
	\subfloat[$\hatlevelset{j+1}$]{\label{fig:biased-density_N}\includegraphics[width=0.2\linewidth]{figures/BFPS/phihat}}\vspace*{-7pt}
	\caption{An example of BFPS in 1D: (a) the level set, $\levelset{j}$; (b) a proposed perturbation, $f^{(j)}$; and (c) the resulting proposed sample, $\hatlevelset{j+1}$.}
	\label{fig:1D-BFPS}
\end{figure}

\highlight{JOHN: do you think I should include more results from the BFPS paper at CVPR?}

We note that the proposed sample, $\hatlevelset{j+1}$ in Figure \ref{fig:1D-BFPS} has undergone a topological change; the small bump on the right is now greater than zero, and the resulting curve contains two connected components. Allowing topological changes is one thing that speeds up the convergence of BFPS. However, in cases where the topology of the object is known, restricting the topology of the curve perturbations can dramatically improve results. This has been shown in the optimization framework of level-set methods initially in \cite{Han2003}, where level set evolution was constrained to not change in (digital) topology. The constraint was extended in \cite{Segonne2008}, where evolution was allowed to change topology, but only by preserving the genus of the curve. We show in the next section how to alter the BFPS framework to control the generated samples to be of any specified topology. We remind the reader that we refer to methods that are constrained to a single topology as single-toplogy methods, and methods that can evolve within a set of allowable topologies as topology-controlled methods.

\subsection{Local Identification of Topology Configurations}
The works of \cite{Han2003} and \cite{Segonne2008} consider the digital topology of the embedded curve of the level-set function based on the topological numbers established in \cite{Bertrand1994}. By reviewing the properties presented in \cite{Bertrand1994} (which extend to other connectivities), we can conclude the resulting topological changes for all pairs of topological numbers. These topologies are shown in Table \ref{tbl:topologies}. We note that in 2D, cavities are the same as handles.
\begin{table}
	\centering
	\begin{tabular}{c c}
		Add pixel to FG & Add pixel to BG\\
		\begin{tabular}{|c||*{3}{c|}}
			\hline
			\backslashbox{$T_{\overline{n}}$}{$T_n$} & $0$ & $1$ & $\geq 2$\\\hline\hline
			\multirow{2}{*}{$0$} 		& \multirow{2}{*}{$\cdot$} 	& FG: DV				& \multirow{2}{*}{$\cdot$} \\
										&							& BG: DR				& \\\hline
			\multirow{2}{*}{$1$} 		& FG: CR					& \multirow{2}{*}{None}	& FG: MR/CH \\
										& BG: CV					& 						& BG: None \\\hline
			\multirow{2}{*}{$\geq 2$}	& \multirow{2}{*}{$\cdot$}	& FG: None				& FG: MR/CH \\
										&							& BG: SR/DH 			& BG: DH/SR \\\hline
		\end{tabular}&
		\begin{tabular}{|c||*{3}{c|}}
			\hline
			\backslashbox{$T_{\overline{n}}$}{$T_n$} & $0$ & $1$ & $\geq 2$\\\hline\hline
			\multirow{2}{*}{$0$} 		& \multirow{2}{*}{$\cdot$} 	& FG: CV				& \multirow{2}{*}{$\cdot$} \\
										&							& BG: CR				& \\\hline
			\multirow{2}{*}{$1$} 		& FG: DR					& \multirow{2}{*}{None}	& FG: SR/DH \\
										& BG: DH					& 						& BG: None \\\hline
			\multirow{2}{*}{$\geq 2$}	& \multirow{2}{*}{$\cdot$}	& FG: None				& FG: SR/DH \\
										&							& BG: MR/CH 			& BG: CH/MR \\\hline
		\end{tabular}
	\end{tabular}
	\caption{Topological changes as a function of topological numbers. Abbreviations: FG - Foreground; BG - Background; C - Create; D - Destroy; S - Split; M - Merge; H - Handle(s); R - Region(s); V - Cavity. Regions are equivalent to connected components. Omitted boxes correspond to impossible topological number pairs.}
	\label{tbl:topologies}
\end{table}

As shown by Segonne \cite{Segonne2008}, distinguishing a split or merge of a region from a creation or destruction of a handle can not be determined solely based on the topological numbers, $T_n$ and $T_{\overline{n}}$. With the extended topological numbers of \cite{Segonne2008}, one is able to distinguish between these topological changes. When a pixel is added to the foreground, $T_n^+=1$ indicates the creation of a handle in the foreground, and $T_{\overline{n}}^+=2$ indicates the merging of regions in the foreground. Similarly, when a pixel is added to the background, $T_n^+=1$ indicates the destruction of a handle in the foreground, and $T_{\overline{n}}^+=2$ indicates the splitting of regions in the foreground.

By labeling each connected component in the foreground and background, Segonne shows that $T_n^+$ can be computed efficiently when a pixel is added to the foreground and $T_{\overline{n}}^+$ when a pixel is added to the background. In 3D, one \textit{must} calculate $T_{overline{n}}^+$ when adding a pixel to the foreground, which can be computationally expensive. We show here that this calculation is not necessary in 2D.

Consider the digital region shown in Figure \ref{fig:handle-id}.
\begin{figure}
	\centering
	\includegraphics[width=0.3\linewidth]{figures/handle_id}
	\caption{Distinguishing between creating splitting a region and removing a handle while moving a pixel is added to the background. Red pixels correspond to the 4-connected foreground. The circle marks the splitting of a region and the triangle marks the destruction of a handle.}
	\label{fig:handle-id}
\end{figure}
We consider two pixels of interest marked by the circle and triangle. Removing the circle pixel from the foreground would result in a splitting of the region, while removing the triangle pixel would result in destroying a handle. Both of these pixels have topological numbers $T_n=2$ and $T_{\overline{n}}=2$. The extended topological numbers, which allow us to distinguish between the topologies, are $T_n^+(\circ)=2$, $T_{\overline{n}}^+(\circ)=1$, $T_n^+(\triangle)=1$, and $T_{\overline{n}}^+(\triangle)=2$. We emphasize here that both $T_n^+$ and $T_{\overline{n}}^+$ are different in this case, which is not necessarily true in 3D. In fact, in 2D, the destruction of a handle in the foreground corresponds directly to a merging of regions in the background, and the splitting of regions in the foreground corresponds directly to a creation of a handle in the background. Because of this one-to-one mapping, we only need to consider $T_{\overline{n}}^+$ when adding a pixel to the background, which can already be computed efficiently.



\begin{comment}
As shown by Segonne \cite{Segonne2008}, distinguishing a split or merge of a region from a creation or destruction of a handle can not be determined solely based on the topological numbers, $T_n$ and $T_{\overline{n}}$. With the extended topological numbers of \cite{Segonne2008}, one is able to distinguish between these topological changes. Segonne, however, only gives an efficient algorithm for determining these extended topological numbers when the components have spherical topology (i.e. no handles). He proposes a simple technique that is able to distinguish merging a region from creating a handle by assigning a unique label to each connected component. We show here how to distinguish between splitting a region and destroying a handle using a local and efficient to an auxillary variable counting the number of the handles, $H$.

We first note that if a region has a handle, removing any single pixel of that region can not split it into two regions; it can only remove the handle. With this in mind, if the number of handles is maintained for each connected component, one can distinguish splitting a region from destroying a handle. With this method, one must be able to compute whether a handle exists in the region. Instead, we maintain a count of the number of handles for each region, as an update to this count is much more efficient than finding this value at every iteration. Given a correct count of previous handles in the foreground and that a pixel is being added to the foreground, the number of handles can be updated by:
\begin{equation}
	H^{(j)} = H^{(j-1)} + T_n - T_n^+.
\end{equation}
Similarly, $T_n^+$ corresponds to the number of regions that will be merged.
\end{comment}

\subsection{Topologically-Controlled Biased Filtered Point Sampling}
Assume that we have a list of topology changes that we would like to allow (e.g. splitting/merging regions), and a set that we would like forbid (changing the genus). We would like to sample from the space of segmentations while honoring this topological constraint. While the goal is similar to \cite{Segonne2008}, a simple alteration of the level-set velocity in an MCMC framework will not preserve detailed balance. One naive approach would be to generate proposals as described in Section \ref{sect:BFPS} and reject any samples that correspond to a forbidden topological change. This is implicitly what the single-topology samplers of \cite{Fan2007} and \cite{Chen2009} do because the forward-backward ratio in their case is zero for \textit{any} topological change. This simple approach, however, will waste a lot of computation time generating samples that are rejected due to their forbidden topology. We take a different approach: only generate proposed samples from the set of allowable topological changes.

Let us first consider a simpler case of only selecting one point for the perturbation and having a filter of finite support and constant height. We draw on the observation that given a filter, $f$, and this one point, $c^{(j)}$, the entire perturbation is completely determined by the value of the Gaussian noise at that point, $n^{(j)}$. Some range of values of $n^{(j)}$ will correspond to allowable topological changes, and some will correspond to forbidden topological changes. If we knew these allowable ranges, we could simply sample from only these ranges.

One naive approach to finding the allowable ranges is to sort all the heights of the window and then consider each range separately. For example, if our filter support contains the heights $\{2, -5, 8\}$, we only need to consider which ranges are allowable among the set $\{(-\infty,-5),(-5,2),(2,8),(8,\infty)\}$. While this will work, we have developed a method for finding the allowable ranges without necessarily having to consider all possible ranges. We exploit the fact that when a forbidden topological change has occured, only certain pixels changing can make it allowable again. For brevity, the details of this search, how to deal with filters of non-constant heights, and how to allow selecting multiple points are not explained here. We refer to this algorithm as topologically-controlled biased filtered point sampling (TC-BFPS).
\begin{comment}
\begin{algorithm}
	\SetAlgoLined
	\KwData{Window of heights, allowable topological changes}
	\KwResult{Allowable ranges}
	
	Fill list \emph{unflipped} with all negative heights\;
	Fill list \emph{onBoundary} with all negative heights bordering positive heights\;
	Sort lists \emph{unflipped} and \emph{onBoundary}\;
	\caption{Finding allowable ranges for positive velocities}
\end{algorithm}
\end{comment}



\subsection{Proposed Work}
While most of the preceding work on sampling shapes has already been completed, some open questions still remain. In this thesis, we will address the following issues:
\begin{enumerate}
	\item Developing fast algorithms for the discovery of allowable proposal regions
	\item Analysis of computational cost using TC-BFPS vs. \cite{Fan2007} or \cite{Chen2009}
	\item Possible extensions to 3D sampling
\end{enumerate}
